Queuing for Secrets: Model-Based Remote Timing Attacks

Remote timing attacks exploit variations in response times to infer sensitive information about remote systems. Their effectiveness, however, is often limited by the difficulty of accurately modeling the stochastic nature of server-side response times, taking into account the intrinsic variability of the service time of a request and the impact of varying workloads on the observed response times. In this article, we propose a new stochastic framework for remote timing attacks based on queuing models and Bayesian statistics. We assume that the attacker knows the service time distributions of two classes of requests and that the information leakage occurs when a malicious observer can distinguish with high probability the class based on the observed response times in the presence of noise induced by exogenous workload. Our experimental evaluation on popular websites demonstrates the practical viability of the approach: our attack outperforms formal techniques based on deterministic service times and existing empirical techniques, while requiring less tuning and fewer hyper-parameters compared to previous formal approaches. Overall, our results show that principled stochastic modeling can provide a solid foundation for building more effective remote timing attacks under realistic network and workload conditions.

==> backup-dituttounpo/firstexps.tex <==
\subsection{Sanity Check with Previous Methodology}


\begin{table}[H]
\centering
\caption{adobe}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.083 & 0.076 & 0.637 & 0.586 & 0.131 & 0.131 & 2 \\ 
\hline
14\_54\_19\_159Z & 0.079 & 0.067 & 0.362 & 0.310 & 0.217 & 0.217 & 2 \\ 
\hline
15\_55\_39\_172Z & 0.093 & 0.092 & 0.570 & 0.566 & 0.162 & 0.162 & 2 \\ 
\hline
16\_56\_59\_180Z & 0.078 & 0.059 & 0.844 & 0.644 & 0.092 & 0.092 & 2 \\ 
\hline
17\_58\_19\_187Z & 0.083 & 0.076 & 0.657 & 0.609 & 0.126 & 0.126 & 2 \\ 
\hline
18\_59\_39\_193Z & 0.079 & 0.070 & 0.290 & 0.257 & 0.273 & 0.273 & 2 \\ 
\hline
20\_00\_59\_199Z & 0.025 & 0.042 & 0.120 & 0.202 & 0.210 & 0.210 & 2 \\ 
\hline
21\_02\_19\_205Z & 0.084 & 0.086 & 0.535 & 0.549 & 0.156 & 0.156 & 2 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_adobe.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_adobe_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{bing}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.052 & 0.022 & 1.931 & 0.810 & 0.027 & 0.027 & 2 \\ 
\hline
14\_54\_19\_159Z & 0.018 & 0.018 & 0.252 & 0.264 & 0.070 & 0.070 & 2 \\ 
\hline
15\_55\_39\_172Z & 0.035 & 0.110 & 0.114 & 0.358 & 0.308 & 0.308 & 2 \\ 
\hline
16\_56\_59\_180Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
17\_58\_19\_187Z & 0.022 & 0.026 & 0.056 & 0.066 & 0.400 & 0.400 & 2 \\ 
\hline
18\_59\_39\_193Z & 0.015 & 0.018 & 0.345 & 0.416 & 0.044 & 0.044 & 2 \\ 
\hline
20\_00\_59\_199Z & 0.017 & 0.021 & 0.367 & 0.439 & 0.047 & 0.047 & 2 \\ 
\hline
21\_02\_19\_205Z & 0.014 & 0.013 & 3.278 & 3.135 & 0.004 & 0.004 & 2 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_bing.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_bing_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{facebook}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 7.398 & 0.348 & 13.744 & 0.647 & 0.538 & 0.538 & 1 \\ 
\hline
14\_54\_19\_159Z & 7.401 & 0.485 & 15.010 & 0.984 & 0.493 & 0.493 & 1 \\ 
\hline
15\_55\_39\_172Z & 9.259 & 0.576 & 52.668 & 3.278 & 0.176 & 0.176 & 1 \\ 
\hline
16\_56\_59\_180Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
17\_58\_19\_187Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
18\_59\_39\_193Z & 9.710 & 0.462 & 21.060 & 1.002 & 0.461 & 0.461 & 1 \\ 
\hline
20\_00\_59\_199Z & 8.205 & 0.595 & 52.652 & 3.821 & 0.156 & 0.156 & 1 \\ 
\hline
21\_02\_19\_205Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_facebook.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_facebook_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{linkedin}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.080 & 0.010 & 0.254 & 0.031 & 0.317 & 0.317 & 3 \\ 
\hline
14\_54\_19\_159Z & 0.072 & 0.010 & 0.206 & 0.029 & 0.351 & 0.351 & 3 \\ 
\hline
15\_55\_39\_172Z & 0.075 & 0.008 & 0.376 & 0.038 & 0.200 & 0.200 & 3 \\ 
\hline
16\_56\_59\_180Z & 0.076 & 0.007 & 0.395 & 0.038 & 0.192 & 0.192 & 3 \\ 
\hline
17\_58\_19\_187Z & 0.073 & 0.010 & 0.208 & 0.029 & 0.351 & 0.351 & 3 \\ 
\hline
18\_59\_39\_193Z & 0.076 & 0.008 & 0.306 & 0.034 & 0.250 & 0.250 & 3 \\ 
\hline
20\_00\_59\_199Z & 0.074 & 0.008 & 0.294 & 0.033 & 0.251 & 0.251 & 3 \\ 
\hline
21\_02\_19\_205Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 3 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_linkedin.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_linkedin_onlyobs.pdf}}\hfill
\end{figure}


\begin{table}[H]
\centering
\caption{live}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.231 & 0.891 & 1259.420 & 4863.835 & 0.000 & 0.000 & 4 \\ 
\hline
14\_54\_19\_159Z & 0.208 & 0.146 & 4.868 & 3.413 & 0.043 & 0.043 & 4 \\ 
\hline
15\_55\_39\_172Z & 0.797 & 2.138 & 1.506 & 4.038 & 0.530 & 0.530 & 4 \\ 
\hline
16\_56\_59\_180Z & 0.751 & 0.748 & 1.119 & 1.114 & 0.671 & 0.671 & 4 \\ 
\hline
17\_58\_19\_187Z & 0.313 & 0.305 & 2.310 & 2.251 & 0.135 & 0.135 & 4 \\ 
\hline
18\_59\_39\_193Z & 0.776 & 3.725 & 1.289 & 6.188 & 0.602 & 0.602 & 4 \\ 
\hline
20\_00\_59\_199Z & 0.301 & 0.289 & 1.413 & 1.356 & 0.213 & 0.213 & 4 \\ 
\hline
21\_02\_19\_205Z & 0.200 & 0.175 & 1.001 & 0.874 & 0.200 & 0.200 & 4 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_live.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_live_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{microsoft}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.003 & 0.008 & 0.090 & 0.222 & 0.036 & 0.036 & 4 \\ 
\hline
14\_54\_19\_159Z & 0.004 & 0.011 & 0.091 & 0.221 & 0.049 & 0.049 & 4 \\ 
\hline
15\_55\_39\_172Z & 0.011 & 0.015 & 0.136 & 0.186 & 0.081 & 0.081 & 4 \\ 
\hline
16\_56\_59\_180Z & 0.029 & 0.029 & 0.226 & 0.226 & 0.128 & 0.128 & 4 \\ 
\hline
17\_58\_19\_187Z & 0.029 & 0.029 & 0.047 & 0.047 & 0.623 & 0.623 & 4 \\ 
\hline
18\_59\_39\_193Z & 0.029 & 0.029 & 0.044 & 0.044 & 0.655 & 0.655 & 4 \\ 
\hline
20\_00\_59\_199Z & 0.029 & 0.029 & 0.049 & 0.049 & 0.600 & 0.600 & 4 \\ 
\hline
21\_02\_19\_205Z & 0.029 & 0.029 & 0.048 & 0.048 & 0.609 & 0.609 & 4 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_microsoft.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_microsoft_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{office}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
14\_54\_19\_159Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
15\_55\_39\_172Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
16\_56\_59\_180Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
17\_58\_19\_187Z & 0.256 & -0.017 & 0.366 & -0.024 & 0.698 & 0.698 & 2 \\ 
\hline
18\_59\_39\_193Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
20\_00\_59\_199Z & 0.192 & 0.061 & 2.419 & 0.772 & 0.079 & 0.079 & 2 \\ 
\hline
21\_02\_19\_205Z & 0.227 & 0.068 & 1.812 & 0.542 & 0.125 & 0.125 & 2 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_office.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_office_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{pinterest}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.003 & 0.013 & 0.076 & 0.314 & 0.040 & 0.040 & 3 \\ 
\hline
14\_54\_19\_159Z & 0.006 & 0.015 & 0.102 & 0.265 & 0.057 & 0.057 & 3 \\ 
\hline
15\_55\_39\_172Z & 0.037 & 0.046 & 0.295 & 0.370 & 0.125 & 0.125 & 3 \\ 
\hline
16\_56\_59\_180Z & 0.005 & 0.012 & 0.090 & 0.210 & 0.057 & 0.057 & 3 \\ 
\hline
17\_58\_19\_187Z & 0.007 & 0.015 & 0.051 & 0.114 & 0.132 & 0.132 & 3 \\ 
\hline
18\_59\_39\_193Z & 0.005 & 0.013 & 0.049 & 0.113 & 0.113 & 0.113 & 3 \\ 
\hline
20\_00\_59\_199Z & 0.005 & 0.018 & 0.104 & 0.411 & 0.044 & 0.044 & 3 \\ 
\hline
21\_02\_19\_205Z & 0.007 & 0.018 & 0.107 & 0.265 & 0.069 & 0.069 & 3 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_pinterest.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_pinterest_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{skype}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.275 & 0.275 & 0.678 & 0.677 & 0.406 & 0.406 & 4 \\ 
\hline
14\_54\_19\_159Z & 0.272 & 0.272 & 0.621 & 0.620 & 0.439 & 0.439 & 4 \\ 
\hline
15\_55\_39\_172Z & 0.017 & 0.079 & 1.692 & 8.055 & 0.010 & 0.010 & 4 \\ 
\hline
16\_56\_59\_180Z & 0.287 & 0.639 & 1.294 & 2.886 & 0.221 & 0.221 & 4 \\ 
\hline
17\_58\_19\_187Z & 0.273 & 0.273 & 0.641 & 0.641 & 0.426 & 0.426 & 4 \\ 
\hline
18\_59\_39\_193Z & 0.206 & 0.288 & 1.492 & 2.086 & 0.138 & 0.138 & 4 \\ 
\hline
20\_00\_59\_199Z & 0.272 & 0.272 & 0.609 & 0.609 & 0.447 & 0.447 & 4 \\ 
\hline
21\_02\_19\_205Z & 0.287 & 0.524 & 1.406 & 2.565 & 0.204 & 0.204 & 4 \\ 
\hline
\end{tabular}
\end{table}


\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_skype.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_skype_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{spotify}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.032 & 0.026 & 0.109 & 0.088 & 0.297 & 0.297 & 4 \\ 
\hline
14\_54\_19\_159Z & 0.032 & 0.027 & 0.113 & 0.096 & 0.286 & 0.286 & 4 \\ 
\hline
15\_55\_39\_172Z & 0.033 & 0.028 & 0.120 & 0.102 & 0.271 & 0.271 & 4 \\ 
\hline
16\_56\_59\_180Z & 0.032 & 0.027 & 0.100 & 0.085 & 0.320 & 0.320 & 4 \\ 
\hline
17\_58\_19\_187Z & 0.032 & 0.020 & 0.157 & 0.101 & 0.202 & 0.202 & 4 \\ 
\hline
18\_59\_39\_193Z & 0.026 & 0.017 & 0.116 & 0.076 & 0.226 & 0.226 & 4 \\ 
\hline
20\_00\_59\_199Z & 0.027 & 0.019 & 0.137 & 0.095 & 0.197 & 0.197 & 4 \\ 
\hline
21\_02\_19\_205Z & 0.025 & 0.014 & 0.168 & 0.090 & 0.151 & 0.151 & 4 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_spotify.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_spotify_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{vimeo}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.361 & 0.614 & 0.745 & 1.267 & 0.485 & 0.485 & 3 \\ 
\hline
14\_54\_19\_159Z & 0.367 & 0.360 & 0.855 & 0.839 & 0.429 & 0.429 & 3 \\ 
\hline
15\_55\_39\_172Z & 0.327 & 0.295 & 0.634 & 0.572 & 0.516 & 0.516 & 3 \\ 
\hline
16\_56\_59\_180Z & 0.364 & 0.353 & 0.799 & 0.775 & 0.456 & 0.456 & 3 \\ 
\hline
17\_58\_19\_187Z & 0.356 & 0.456 & 0.681 & 0.872 & 0.523 & 0.523 & 3 \\ 
\hline
18\_59\_39\_193Z & 0.297 & 0.259 & 0.685 & 0.596 & 0.434 & 0.434 & 3 \\ 
\hline
20\_00\_59\_199Z & 0.359 & 0.466 & 0.714 & 0.928 & 0.502 & 0.502 & 3 \\ 
\hline
21\_02\_19\_205Z & 0.345 & 0.285 & 0.989 & 0.817 & 0.348 & 0.348 & 3 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_vimeo.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_vimeo_onlyobs.pdf}}\hfill
\end{figure}

\begin{table}[H]
\centering
\caption{wikipedia}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.008 & 0.004 & 0.374 & 0.185 & 0.021 & 0.021 & 4 \\ 
\hline
14\_54\_19\_159Z & 0.009 & 0.004 & 0.403 & 0.151 & 0.023 & 0.023 & 4 \\ 
\hline
15\_55\_39\_172Z & 0.008 & 0.004 & 0.159 & 0.087 & 0.049 & 0.049 & 4 \\ 
\hline
16\_56\_59\_180Z & 0.009 & 0.005 & 0.105 & 0.053 & 0.089 & 0.089 & 4 \\ 
\hline
17\_58\_19\_187Z & 0.009 & 0.004 & 0.161 & 0.076 & 0.055 & 0.055 & 4 \\ 
\hline
18\_59\_39\_193Z & 0.008 & 0.004 & 0.238 & 0.124 & 0.032 & 0.032 & 4 \\ 
\hline
20\_00\_59\_199Z & 0.011 & 0.004 & 0.156 & 0.065 & 0.068 & 0.068 & 4 \\ 
\hline
21\_02\_19\_205Z & 0.009 & 0.004 & 0.168 & 0.076 & 0.053 & 0.053 & 4 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_wikipedia.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_wikipedia_onlyobs.pdf}}\hfill
\end{figure}


\begin{table}[H]
\centering
\caption{x}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.198 & 0.128 & 1.941 & 1.253 & 0.102 & 0.102 & 4 \\ 
\hline
14\_54\_19\_159Z & 0.209 & 0.130 & 2.029 & 1.263 & 0.103 & 0.103 & 4 \\ 
\hline
15\_55\_39\_172Z & 0.149 & 0.105 & 1.856 & 1.310 & 0.080 & 0.080 & 4 \\ 
\hline
16\_56\_59\_180Z & 0.343 & 0.176 & 4.144 & 2.122 & 0.083 & 0.083 & 4 \\ 
\hline
17\_58\_19\_187Z & 0.142 & 0.120 & 1.735 & 1.470 & 0.082 & 0.082 & 4 \\ 
\hline
18\_59\_39\_193Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 4 \\ 
\hline
20\_00\_59\_199Z & 0.114 & 0.080 & 4.534 & 3.172 & 0.025 & 0.025 & 4 \\ 
\hline
21\_02\_19\_205Z & 0.143 & 0.099 & 3.769 & 2.601 & 0.038 & 0.038 & 4 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_x.pdf}}\hfill
  \subfloat[]{\includegraphics[width=0.49\linewidth]{plots/comparison_x_onlyobs.pdf}}\hfill
\end{figure}




==> backup-dituttounpo/firstexps_mode_shift_ps.tex <==


\begin{table}[H]
\centering
\caption{adobe}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.083 & 0.106 & 0.637 & 0.786 & 0.131 & 0.135 & 2 \\ 
\hline
14\_54\_19\_159Z & 0.079 & 0.092 & 0.362 & 0.418 & 0.217 & 0.221 & 2 \\ 
\hline
15\_55\_39\_172Z & 0.093 & 0.130 & 0.570 & 0.783 & 0.162 & 0.166 & 2 \\ 
\hline
16\_56\_59\_180Z & 0.078 & 0.083 & 0.844 & 0.866 & 0.092 & 0.096 & 2 \\ 
\hline
17\_58\_19\_187Z & 0.083 & 0.108 & 0.657 & 0.836 & 0.126 & 0.130 & 2 \\ 
\hline
18\_59\_39\_193Z & 0.079 & 0.095 & 0.290 & 0.343 & 0.273 & 0.277 & 2 \\ 
\hline
20\_00\_59\_199Z & 0.025 & 0.053 & 0.120 & 0.248 & 0.210 & 0.213 & 2 \\ 
\hline
21\_02\_19\_205Z & 0.084 & 0.118 & 0.535 & 0.737 & 0.156 & 0.160 & 2 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_adobe_modeShift.pdf}
\end{figure}

\begin{table}[H]
\centering
\caption{bing}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.052 & 0.025 & 1.931 & 0.877 & 0.027 & 0.028 & 2 \\ 
\hline
14\_54\_19\_159Z & 0.018 & 0.016 & 0.252 & 0.229 & 0.070 & 0.071 & 2 \\ 
\hline
15\_55\_39\_172Z & 0.035 & 0.017 & 0.114 & 0.055 & 0.308 & 0.308 & 2 \\ 
\hline
16\_56\_59\_180Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
17\_58\_19\_187Z & 0.022 & 0.026 & 0.056 & 0.066 & 0.400 & 0.400 & 2 \\ 
\hline
18\_59\_39\_193Z & 0.015 & 0.018 & 0.345 & 0.401 & 0.044 & 0.045 & 2 \\ 
\hline
20\_00\_59\_199Z & 0.017 & 0.021 & 0.367 & 0.437 & 0.047 & 0.048 & 2 \\ 
\hline
21\_02\_19\_205Z & 0.014 & 0.012 & 3.278 & 2.404 & 0.004 & 0.005 & 2 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_bing_modeShift.pdf}
\end{figure}


\begin{table}[H]
\centering
\caption{facebook}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 7.398 & 0.257 & 13.744 & 0.361 & 0.538 & 0.711 & 2 \\ 
\hline
14\_54\_19\_159Z & 7.401 & 0.499 & 15.010 & 0.730 & 0.493 & 0.683 & 2 \\ 
\hline
15\_55\_39\_172Z & 9.259 & 0.586 & 52.668 & 1.208 & 0.176 & 0.485 & 2 \\ 
\hline
16\_56\_59\_180Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 2 \\ 
\hline
17\_58\_19\_187Z & 0.000 & 0.907 & 0.000 & 3.986 & NaN & 0.228 & 2 \\ 
\hline
18\_59\_39\_193Z & 9.710 & 0.481 & 21.060 & 0.725 & 0.461 & 0.663 & 2 \\ 
\hline
20\_00\_59\_199Z & 8.205 & 0.630 & 52.652 & 1.333 & 0.156 & 0.472 & 2 \\ 
\hline
21\_02\_19\_205Z & 0.000 & 1.037 & 0.000 & 61.522 & NaN & 0.017 & 2 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_facebook_modeShift.pdf}
\end{figure}


\begin{table}[H]
\centering
\caption{live}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.231 & 0.110 & 1259.420 & 2.394 & 0.000 & 0.046 & 2 \\ 
\hline
14\_54\_19\_159Z & 0.208 & 0.280 & 4.868 & 3.227 & 0.043 & 0.087 & 2 \\ 
\hline
15\_55\_39\_172Z & 0.797 & 3.609 & 1.506 & 6.548 & 0.530 & 0.551 & 2 \\ 
\hline
16\_56\_59\_180Z & 0.751 & 0.777 & 1.119 & 1.133 & 0.671 & 0.686 & 2 \\ 
\hline
17\_58\_19\_187Z & 0.313 & 0.554 & 2.310 & 3.165 & 0.135 & 0.175 & 2 \\ 
\hline
18\_59\_39\_193Z & 0.776 & 0.803 & 1.289 & 1.295 & 0.602 & 0.620 & 2 \\ 
\hline
20\_00\_59\_199Z & 0.301 & 0.404 & 1.413 & 1.623 & 0.213 & 0.249 & 2 \\ 
\hline
21\_02\_19\_205Z & 0.200 & 0.276 & 1.001 & 1.166 & 0.200 & 0.236 & 2 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_live_modeShift.pdf}
\end{figure}


\begin{table}[H]
\centering
\caption{microsoft}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.003 & 0.015 & 0.090 & 0.161 & 0.036 & 0.090 & 6 \\ 
\hline
14\_54\_19\_159Z & 0.004 & 0.109 & 0.091 & 1.067 & 0.049 & 0.102 & 6 \\ 
\hline
15\_55\_39\_172Z & 0.011 & 0.165 & 0.136 & 1.239 & 0.081 & 0.133 & 6 \\ 
\hline
16\_56\_59\_180Z & 0.029 & 0.035 & 0.226 & 0.196 & 0.128 & 0.177 & 6 \\ 
\hline
17\_58\_19\_187Z & 0.029 & 0.030 & 0.047 & 0.047 & 0.623 & 0.644 & 6 \\ 
\hline
18\_59\_39\_193Z & 0.029 & 0.030 & 0.044 & 0.045 & 0.655 & 0.675 & 6 \\ 
\hline
20\_00\_59\_199Z & 0.029 & 0.031 & 0.049 & 0.050 & 0.600 & 0.622 & 6 \\ 
\hline
21\_02\_19\_205Z & 0.029 & 0.031 & 0.048 & 0.049 & 0.609 & 0.631 & 6 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_microsoft_modeShift.pdf}
\end{figure}


\begin{table}[H]
\centering
\caption{office}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
14\_54\_19\_159Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
15\_55\_39\_172Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
16\_56\_59\_180Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
17\_58\_19\_187Z & 0.256 & 0.001 & 0.366 & 0.001 & 0.698 & 0.677 & 1 \\ 
\hline
18\_59\_39\_193Z & 0.000 & 0.000 & 0.000 & 1.000 & NaN & 0.000 & 1 \\ 
\hline
20\_00\_59\_199Z & 0.192 & 0.053 & 2.419 & 3.483 & 0.079 & 0.015 & 1 \\ 
\hline
21\_02\_19\_205Z & 0.227 & 0.060 & 1.812 & 0.933 & 0.125 & 0.064 & 1 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_office_modeShift.pdf}
\end{figure}


\begin{table}[H]
\centering
\caption{pinterest}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.003 & 0.101 & 0.076 & 1.332 & 0.040 & 0.076 & 6 \\ 
\hline
14\_54\_19\_159Z & 0.006 & 0.106 & 0.102 & 1.155 & 0.057 & 0.092 & 6 \\ 
\hline
15\_55\_39\_172Z & 0.037 & 0.042 & 0.295 & 0.267 & 0.125 & 0.158 & 6 \\ 
\hline
16\_56\_59\_180Z & 0.005 & 0.083 & 0.090 & 0.901 & 0.057 & 0.092 & 6 \\ 
\hline
17\_58\_19\_187Z & 0.007 & 0.100 & 0.051 & 0.606 & 0.132 & 0.165 & 6 \\ 
\hline
18\_59\_39\_193Z & 0.005 & 0.055 & 0.049 & 0.375 & 0.113 & 0.146 & 6 \\ 
\hline
20\_00\_59\_199Z & 0.005 & 0.199 & 0.104 & 2.497 & 0.044 & 0.080 & 6 \\ 
\hline
21\_02\_19\_205Z & 0.007 & 0.128 & 0.107 & 1.231 & 0.069 & 0.104 & 6 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_pinterest_modeShift.pdf}
\end{figure}


\begin{table}[H]
\centering
\caption{spotify}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.032 & 0.177 & 0.109 & 0.441 & 0.297 & 0.401 & 5 \\ 
\hline
14\_54\_19\_159Z & 0.032 & 0.199 & 0.113 & 0.506 & 0.286 & 0.392 & 5 \\ 
\hline
15\_55\_39\_172Z & 0.033 & 0.203 & 0.120 & 0.535 & 0.271 & 0.379 & 5 \\ 
\hline
16\_56\_59\_180Z & 0.032 & 0.192 & 0.100 & 0.455 & 0.320 & 0.421 & 5 \\ 
\hline
17\_58\_19\_187Z & 0.032 & 0.166 & 0.157 & 0.518 & 0.202 & 0.320 & 5 \\ 
\hline
18\_59\_39\_193Z & 0.026 & 0.116 & 0.116 & 0.341 & 0.226 & 0.341 & 5 \\ 
\hline
20\_00\_59\_199Z & 0.027 & 0.146 & 0.137 & 0.462 & 0.197 & 0.317 & 5 \\ 
\hline
21\_02\_19\_205Z & 0.025 & 0.109 & 0.168 & 0.394 & 0.151 & 0.277 & 5 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_spotify_modeShift.pdf}
\end{figure}



\begin{table}[H]
\centering
\caption{vimeo}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.361 & 0.380 & 0.745 & 0.808 & 0.485 & 0.470 & 1 \\ 
\hline
14\_54\_19\_159Z & 0.367 & 0.260 & 0.855 & 0.631 & 0.429 & 0.413 & 1 \\ 
\hline
15\_55\_39\_172Z & 0.327 & 0.238 & 0.634 & 0.474 & 0.516 & 0.502 & 1 \\ 
\hline
16\_56\_59\_180Z & 0.364 & 0.248 & 0.799 & 0.565 & 0.456 & 0.440 & 1 \\ 
\hline
17\_58\_19\_187Z & 0.356 & 0.320 & 0.681 & 0.628 & 0.523 & 0.509 & 1 \\ 
\hline
18\_59\_39\_193Z & 0.297 & 0.207 & 0.685 & 0.495 & 0.434 & 0.418 & 1 \\ 
\hline
20\_00\_59\_199Z & 0.359 & 0.305 & 0.714 & 0.625 & 0.502 & 0.488 & 1 \\ 
\hline
21\_02\_19\_205Z & 0.345 & 0.207 & 0.989 & 0.629 & 0.348 & 0.329 & 1 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_vimeo_modeShift.pdf}
\end{figure}


\begin{table}[H]
\centering
\caption{x}
\begin{tabular}{|c|cc|cc|cc|c|}
\hline
\multirow{2}{*}{Exp ID} & \multicolumn{2}{c|}{$\lambda$} & \multicolumn{2}{c|}{$\mu$} & \multicolumn{2}{c|}{$\rho$} & \multirow{2}{*}{k0} \\ 
 & D & C & D & C & D & C & \\ 
\hline
13\_52\_59\_146Z & 0.198 & 3.347 & 1.941 & 12.270 & 0.102 & 0.273 & 9 \\ 
\hline
14\_54\_19\_159Z & 0.209 & 0.730 & 2.029 & 2.670 & 0.103 & 0.273 & 9 \\ 
\hline
15\_55\_39\_172Z & 0.149 & 1.767 & 1.856 & 6.916 & 0.080 & 0.255 & 9 \\ 
\hline
16\_56\_59\_180Z & 0.343 & 0.733 & 4.144 & 2.848 & 0.083 & 0.257 & 9 \\ 
\hline
17\_58\_19\_187Z & 0.142 & 2.522 & 1.735 & 9.832 & 0.082 & 0.257 & 9 \\ 
\hline
18\_59\_39\_193Z & 0.000 & 1.187 & 0.000 & 6.237 & NaN & 0.190 & 9 \\ 
\hline
20\_00\_59\_199Z & 0.114 & 0.884 & 4.534 & 4.197 & 0.025 & 0.211 & 9 \\ 
\hline
21\_02\_19\_205Z & 0.143 & 0.283 & 3.769 & 1.282 & 0.038 & 0.221 & 9 \\ 
\hline
\end{tabular}
\end{table}

\begin{figure}[H]
  \centering
  \includegraphics[width=0.49\linewidth]{plots/comparison_x_modeShift.pdf}
\end{figure}


==> backup-dituttounpo/mm1fcfs.tex <==
\subsection{Response time distribution in M/M/1/FCFS with a probe job}




Let $\wrv$ be the r.v. associated with the stationary waiting time of an arbitrary job.
We know that under the stability condition $\rho<1$, the CDF of this r.v. can be expressed in the following way:
\[
\wcdf(t)=Prob\{\wrv \leq t\}\,.
\]


Then, we can define the Laplace-Stieltjes transform:
\[
\wlst(s)\triangleq\int_0^\infty \exp(-s t) d_tW(t)
\]
of the equilibrium waiting time distribution: 
\begin{equation}\label{eq:conditional.fcfs}
\wlst(s) = \dfrac{\mu-\lambda}{s+\mu-\lambda}\,.
\end{equation}

Let $\xcdf(\tau)$ be the CDF of the service time distribution of the probe job and $\xlst(s)$ its Laplace transform. Then, the Laplace transform of its response time is: 
\begin{equation}\label{eq:lst-resptime-fcfs}
    \rlst(s) = \xlst(s)\cdot \xlst(s) = \wlst(s)\dfrac{\mu-\lambda}{s+\mu-\lambda}\,,
\end{equation}


\noindent we can state Theorem~\ref{th:probe-erl-fcfs}.

\begin{theorem}\label{th:probe-erl-fcfs}
    Given a M/M/1/FCFS queueing system with $\rho < 1$, assume that a probe job has a service time distributed according to an Erlang-k r.v. with $k\gamma$ being the rate at each Erlang phase, and the Erlang parameter and itself. Then, the Laplace-Stieltjes transform of the probe job's response time is:
    \begin{equation}\label{eq:fcfs.response.transform.erl}
        \rlst(s) = \left(\dfrac{k\gamma}{k\gamma+s}\right)^k\dfrac{\mu-\lambda}{s+\mu-\lambda}
    \end{equation}
    and we can symbolically invert it as (\textcolor{red}{AND WE OBTAIN THE FOLLOWING \underline{PDF}!!}:
\begin{multline}\label{eq:fcfs.response.invtransform.erl}
        \rpdf(t) = \exp(-t(\lambda+\mu))\left(\dfrac{k \gamma}{k\gamma -\lambda + \mu}\right)^k (\lambda-\mu)\cdot \\ \cdot \left(1-\exp(-k\gamma +\lambda - \mu)\sum_{\ell=0}^{k-1} \dfrac{(k\gamma -\lambda +\mu)^{\ell}}{\ell !}\right)
    \end{multline}
\end{theorem}





\subsection{Parameter Estimation}
\begin{comment}
In order to do so we first make the following observations (\textcolor{red}{evitare s fa confusione con la s delle trasformate}):
\[
Pr\{\wrv=0 | \xrv=p,\ \rrv=q \} = \mathds{1}_{q\leq p}\,,
\]
we decondition with respect to the service time distribution
\begin{align*}
Pr\{\wrv=0 | \rrv=q \} &= \int_0^{\infty} \mathds{1}_{q\leq p} \xpdf(p) dp\\ & = \int_r^\infty \xlst(p) dp = 1-\xcdf(q)\,,
\end{align*}

the last step consists of deconditioning with respect to the discrete amount of response time observations, so to obtain:
\begin{align*}
\widehat{Pr}\{\wrv=0\}&=1-\dfrac{1}{N^R}\sum_{i=1}^{N^R} \xcdf(r_i, k, \gamma)\\ &= 1-\dfrac{1}{N^R}\sum_{i=1}^{N^R}\vcdf(r_i - C, k, \gamma)\,.
\end{align*}
\end{comment}
We compute $\widehat{Pr}\{\wrv=0\}$ as before.

Now, recalling that in M/M/1/FCFS queuing system, the expected response time of a customer with an arbitrary service time is 
\[
E[\rrv] = \dfrac{1}{\mu-\lambda} =  \dfrac{1/\mu}{1-\rho} = \overline{Y^R}\,,
\]
that the probability of finding the system empty is
\[
\pi_0 = 1 -\rho\,,
\]
and observing that: 
\[
\widehat{\pi_0} = \widehat{Pr}\{\wrv=0\}
\]
On the basis of these observation, we obtain the estimated load factor as:
\[
\widehat{\rho} = 1 - \widehat{Pr}\{\wrv=0\}\,,
\]
and the estimated service rate as
\[
\widehat{\mu} = \dfrac{1}{\overline{Y^R}\widehat{\pi_0}}\,.
\]




==> backup-dituttounpo/mm1ps.tex <==
\subsection{Response time distribution in M/M/1/PS with probe job}
\textcolor{blue} {Io qui' aggiungerei una prima descrizione qualitativa del metodo seguito per ottenere il risultato desiderato 
\begin{itemize}
\item richiamando e commentando minimamente il risultato di Muntz, Coffman etc\\
\item evidenziando la necessita' di completare quel risultato per ottenere il Response time
\item motivando la scelta di ottenere il risultato desiderato inserendo il probe job\
\item e quindi spiegando il ruolo dei corollari e del teorema\\
\end{itemize}
\ \\
\ \\
}
With a slight abuse of notation, we define the following expressions to facilitate the subsequent discussion.
\begin{align*}
    a &= \lambda(1-\muntzroot)\\
    b &= (1-\rho \muntzroot)^2\\
    g &= \rho (1-\muntzroot)^2\\
    h &= \dfrac{\mu (1-\rho \muntzroot^2)}{\muntzroot}
\end{align*}

where $\muntzroot$ is the smallest of the two positive roots of the equation
\[
\rho \muntzroot^2 - (\lambda + \mu + s) \muntzroot + \mu = 0
\]
The expression for $\muntzroot$ is the following
\[
\muntzroot = \dfrac{\lambda + \mu + s - [(\lambda+\mu+s)^2 - 4 \mu\lambda]^{1/2}}{2\lambda},\ \text{and}\ \rho=\dfrac{\lambda}{\mu}<1\,.
\]
Notice that $\lambda,\ \mu \in  \mathbb{R^+}$, moreover as stated in~\cite{morrison}, $0 < \muntzroot \leq 1,\ \text{for}\ s\geq 0\,.$


Let $\mathcal W_\eta$ be the r.v. associated with the stationary waiting time of a job whose service requirement is $\eta$.
From \cite[Corollary 1]{muntz-lstPSwaitTime} we know that under the stability condition $\rho<1$, the CDF of this r.v. can be expressed in the following way:
\[
\wcdf(\eta, t)=Prob\{\mathcal \wrv_\eta \leq t\}\,.
\]


Then, we can define the Laplace-Stieltjes transform:
\[
\wlst(\eta,s)\triangleq\int_0^\infty \exp(-s t) d_t\wcdf(\eta,t)
\]
of the equilibrium waiting time distribution conditioned on the job requiring $\eta$ units of service, namely  

\begin{equation}\label{eq:conditional.ps}
\wlst(\eta, s) = \dfrac{(1-\rho)(1-\rho \muntzroot^2)\exp(- a \eta)}{b - g \cdot \exp(-h\eta)}\,.
\end{equation}

with $\eta \in \mathbb R^+$ representing the deterministic service time of the probe job. 
Let $\rrv_\eta$ be the r.v. associated with a job of size $\eta$, and let $\rcdf(\eta,t)$ be the corresponding CDF defined as: 
\[
\rcdf(\eta,t)=
\begin{cases}
0 & \text{if }t < \eta \\
\wcdf(\eta, t-\eta) & t \geq \eta
\end{cases}
\]
i.e., the CDFs of $\rrv_\eta$ and $\wrv_\eta$ are the same modulo a shifting on the $t$-axis of width $\eta$.
\[
\wcdf(\eta, t) = \rcdf(\eta, t+\eta)\,, \quad t\geq \eta 
\]



Applying the \textit{time-shifting} property of Laplace transforms\footnote{Given the function $f(t)$ and its respective Laplace transform $f^*(s)$ we have that \[f(t-a)u(t-a)=\exp(-a s) f^*(s)\,.\]}, we obtain the Laplace transform of the response time, conditioned on the job requiring a service time $\eta$:
\begin{equation}\label{eq:shift}
\rlst(\eta, s) = \exp(-s \eta) \wpdf(\eta, s)\,.
\end{equation}
\begin{itemize}
\item \textcolor{red}{Chiarire bene che $\eta$ è una quantità deterministica, e $\tau$ invece è un parametro di una distribuzione, entrambi riferiti al service time del probe job}
\item \textcolor{red}{abbiamo la trasformata condsizionata su un $\tau$, poi passiamo a dare una distribuzione a questo probe job. Di fatto asusmiamo che questo probe job non alteri il funzionamento del sistema in quanto è un uno su infiniti, che arriva e vede il sistema come se lui non ci fosse e vede successivamente il sistema alterttando inalterato}
\end{itemize}
By the law of total probabilities we can decondition the expression above as follows:
\begin{equation}\label{eq:totprob}
    \rlst(s) = \int_0^\infty \rlst(\tau, s) d\xcdf(\tau)\,,
\end{equation}
where $\xcdf(\tau)$ is the CDF of the service time distribution of the probe job. 


\noindent Given the following definition

\begin{definition}
    The Lerch Trascendent function~\cite[Eq.~(25.14.1), pp. 612]{nist} is defined as:
    \[
    \Phi(z,u,\alpha) = \sum_{n=0}^{\infty} \dfrac{z^n}{(\alpha+n)^u}\,, \quad \text{with } |z|<1\,,
    \]
    which converges for any real number $\alpha>0$, where $|z|<1$, or $\mathrm{Re}(u) > 1$, and $|z| = 1$\,.
\end{definition}

\noindent we can state Theorem~\ref{th:probe-erl}.




\begin{theorem}\label{th:probe-erl}
    Given a M/M/1/PS (\textcolor{red}{NB. chiarire che caratterizzando il service time del probe job con una Erlang-k non stiamo andando a studiare una M/Erl/1/PS}) queueing system with $\rho < 1$, assume that a probe job has a service time distributed according to an Erlang-k r.v. \textcolor{red}{with $k\gamma$ being the rate at each Erlang phase, and the Erlang parameter and itself}. Then, the Laplace-Stieltjes transform of the probe job's response time is:
    \begin{equation}\label{eq:ps.response.transform.erl}
        \rlst(s) = (k\gamma)^k(1-\rho)(1-\rho \muntzroot^2) \dfrac{1}{bh^k}\Phi\left(\dfrac{g}{b}, k, \dfrac{s+a+k\gamma}{h}\right)
    \end{equation}
\end{theorem}

In order to prove Theorem~\ref{th:probe-erl}, we need to state and prove the following two lemmas.

\begin{lemma}\label{lem:geomseries}
\[
    \dfrac{1}{1-\dfrac{g}{b}\exp(-h\tau)} =\sum_{n=0}^{\infty} \dfrac{g}{b}\exp(-h\tau)\,,
\]
as $\left|\dfrac{g}{b}\exp(-h\tau)\right|<1$, by Lemma~\ref{lem:bcg1}, and since $h,\ \tau \in \mathbb{R}^+$\\
(\textcolor{red}{E' giusto che l'argomento della sommatoria in $n$ non dipenda da $n$?  Inoltre, dove usiamo il Lemma 1 nella dimostrazine del teorema 1?})

\end{lemma}
% trasformata waiting time
% essendo il R = W + tau posso fare shift nel tempo della trasformata e ottengo trasformata resp time
% ora con legge total prob decondiziono per ottenere R medio decondizionato e aggiungo tempo servizio esponenziale con parametro gamma (?) problemito ?

\begin{lemma}\label{lem:changeOfVar}
We have that
\[
\int_0^{\infty} t^{k-1} \exp(-p t)\ d t = \dfrac{\Gamma(k)}{p^k}
\]    
\end{lemma}
\begin{proof}
\begin{align*}
    \int_0^{\infty} t^{k-1} \exp(-p t)\ d t &= \int_0^{\infty} \left(\dfrac{u}{p}\right)^{k-1} \dfrac{\exp(-u)}{p} \ \ d u \\ &\quad \text{by variable change } u = p t\\
    &= \dfrac{1}{p^k} \int_0^{\infty} u^{k-1} \exp(-u)\ d u\quad \\ &\text{pulling out constant factors}\\
    &= \dfrac{\Gamma(k)}{p^k}\quad \text{by integral repr.}\\ &\text{of Gamma function}
\end{align*}
\end{proof}

We are now in the condition of proving Theorem~\ref{th:probe-erl} as follows.






\begin{definition}
    The Hypergeometric function~\cite[Eq.~(15.2.1), pp. 384]{nist}, $_2F_1(k,y;u;z)$ is defined as:
    \[
    _2F_1(m,p;u;z) = \sum_{n=0}^{\infty} \dfrac{(m)_n (p)_n}{(u)_n}\dfrac{z^n}{n!}\,, \quad \text{ with } |z|<1,\ u > 0,\ 
    \]
    with $(q)_n$ being the (rising) Pochhammer symbol\footnote{Pochhammer symbol $(q)_n$ is defined as follows:
    \[
    (q)_n = \begin{cases}
        1 & n =0\\
        q(q+1)\cdots (q+n-1) & n > 0
    \end{cases}
    \]} and considering it converges conditionally when $-1<\mathrm{Re}(u-m-p)\leq 0\,.$ and $z=1$ is excluded.
\end{definition}



\begin{comment}
\noindent Given the following definitions and :
\begin{itemize}
    \item the Lerch Trascendent function~\cite[Eq.~(25.14.1), pp. 612]{nist}:
    \[
    \Phi(z, v,y) = \sum_{n=0}^{\infty} \dfrac{z^n}{(y+n)^v}\,, \quad \text{with } |z|<1\,,
    \]
    which converges for any real number $y>0$, where $|z|<1$, or $\mathcal{R}(s) > 1$, and $|z| = 1$\,.
    \item the hypergeometric function~\cite[Eq.~(15.2.1), pp. 384]{nist}:
    \[
    _2F_1(k,y;v;z) = \sum_{n=0}^{\infty} \dfrac{(k)_n (y)_n}{(v)_n}\dfrac{z^n}{n!}\,, \quad \text{with} |z|<1,\ v > 0,\ 
    \]
    with $(q)_n$ being the (rising) Pochhammer symbol\footnote{Pochhammer symbol $(q)_n$ is defined as follows:
    \[
    (q)_n = \begin{cases}
        1 & n =0\\
        q(q+1)\cdots (q+n-1) & n > 0
    \end{cases}
    \]} and considering it converges conditionally when $-1<\mathcal{R}(v-k-y)\leq 0\,.$ and $z=1$ is excluded.
    % \item We also have:
    % \[
    % _2F_1(k, y;v, z) =\ _2F_1(y, k;v, z)\,, 
    % \]
    % by symmetry of the inferior indices.
    \item We also have a connection of the Lerch Trascendent function with the hypergeoemtric function:
    \[
    \Phi(z,1,y)=\dfrac{_2F_1(1, y, y+1, z)}{y}\,, \quad |z| < 1
    \]
    From~\cite[Eq.~(9.559), pp. 1039]{zwillinger2007table}
\end{itemize}
\end{comment}





\begin{result}\label{res:relationHyperLerch}
    We also have a connection of the Lerch Trascendent function with the hypergeomtric function:
    \[
    \Phi(z,1,\alpha)=\dfrac{_2F_1(1, \alpha, \alpha+1, z)}{\alpha}\,, \quad |z| < 1
    \]
    From~\cite[Eq.~(9.559), pp. 1039]{zwillinger2007table}
\end{result}

\begin{lemma}[Existance and Convergence]\label{lem:bcg1}      
The function
\[
_2F_1\left(1, \dfrac{a+\gamma +s}{h}; \dfrac{a+h+\gamma +s}{h}; \dfrac{g}{b} \right)
\]
exists and converges (conditionally) if and only if the following conditions are satisfied.
\[
\mathrm{(i)}\ \left|\dfrac{g}{b}\right| < 1\,,\ \mathrm{(ii)} \ \dfrac{s+a+\gamma+h}{h} > 0\,,\ 
\]
\[
\mathrm{(iii)}\ -1<\mathrm{Re}\left(\dfrac{s+a+\gamma+h}{h}-1-\dfrac{s+a+\gamma}{h}\right)\leq 0
\]
\end{lemma}
\begin{proof}
    We prove the three conditions separately.\\
    
    \noindent $\mathrm{(i)}$ $\left|\dfrac{g}{b}\right| < 1$\\
    \begin{align*}
        \dfrac{\rho(1-\muntzroot)^2}{(1-\rho \muntzroot)^2} &< 1\\
        \rho(1-\muntzroot)^2 &< (1-\rho \muntzroot)^2\\
        \rho(1-2\muntzroot+\muntzroot^2) &< (1-2\rho \muntzroot + \rho^2 \muntzroot^2) \\
        \rho +\rho \muntzroot^2 -1 -\rho^2 \muntzroot^2 &< 0\\
        \rho -1 + \rho \muntzroot^2 (1-\rho) &< 0\\
        (\rho -1) (1-\rho \muntzroot^2) &< 0
    \end{align*}
    since $0<\rho<1$, we have $(\rho -1)<0$, thus the inequality holds if 
    \[
    1-\rho \muntzroot^2 > 0,\quad  \text{i.e.,}\quad \muntzroot^2 <\dfrac{1}{\rho}
    \]
    as $0<\muntzroot\leq 1$ we need $1\leq \rho^{-1}$ which is always true for $0< \rho<1$. Thus, Condition (i) is satisfied.\\
    
    \noindent $\mathrm{(ii)}$ $\dfrac{s+a+\gamma+h}{h} > 0$\\
    \begin{itemize}
        \item[] $s\geq 0$, $\gamma > 0$
        \item[] $a = \lambda(1-\muntzroot)$, since $\lambda > 0$ and $0<\muntzroot\leq 1$ we obtain $a \geq 0$
        \item[] $h = \dfrac{\mu(1-\rho \muntzroot^2)}{\muntzroot}>0$, since $0<\muntzroot\leq 1$, $\mu > 0$, and $0<\rho<1$
    \end{itemize}
    Hence, condition $\mathrm{(ii)}$ is satisfied\\

    \noindent $\mathrm{(iii)}$ $\mathrm{Re}\left(\dfrac{s+a+\gamma+h}{h}-1-\dfrac{s+a+\gamma}{h}\right)\leq 0$\\
    
    After few algebraic steps we notice that the expression above is equal 0, thus condition (iii) is satisfied.\\
\end{proof}

\begin{corollary}\label{cor:mm1psexp}
    Given a M/M/1/PS queueing system with $\rho < 1 $, assume that a probe job has a service time distributed according to an Exponential r.v. Then, the Laplace-Stieltjes transform of the probe job's response time is:
    {\small
    \begin{equation}
        \rlst(s) = \dfrac{\gamma(1-\rho)(1-\rho \muntzroot^2)\ _2F_1\left(1, \dfrac{a+\gamma +s}{h}; \dfrac{a+h+\gamma +s}{h}; \dfrac{g}{b} \right)}{b(a+\gamma+s)}
    \end{equation}}
\end{corollary}



%Add here Muntz's result and our result on M/M/1/PS with probe job with Erlang service time distribution.
\begin{comment}
\begin{theorem}
Given a M/M/1/PS queueing system with $\rho<1$, assume that a probe job  has a service time distributed according to an Erlang-$k$ r.v.. Then, the Laplace-Stieltjes transform of the probe job's response time is:

\begin{multline}\label{eq:ps.response.transform}
\, _2F_1\left(1,\frac{x (\lambda (x-1)-s-\mu)}{\lambda x^2-\mu};-\frac{\mu + x (\lambda - 2 \lambda x + s + \mu)}{\lambda x^2 - \mu};\frac{\lambda (x-1)^2 \mu}{(\mu-\lambda x)^2}\right)\\ \cdot \frac{1}{(1-x \rho)^2 (\lambda(1-x)+s+u)}
\end{multline}


\begin{multline}\label{eq:ps.response.transform.exp}
\, _2F_1\left(1,\frac{x (\lambda (x-1)-s-\mu)}{\lambda x^2-\mu};-\frac{\mu + x (\lambda - 2 \lambda x + s + \mu)}{\lambda x^2 - \mu};\frac{\lambda (x-1)^2 \mu}{(\mu-\lambda x)^2}\right)\\ 
\cdot \dfrac{(1-\rho)(1-\rho x^2)\mu}{(1-x \rho)^2 (\lambda(1-x)+s+u)}
\end{multline}
When $k=1$, i.e. when the Erlang distribution collapses in an exponential distribution. The LST of the probe job's response time with an arbitrary number of phases $k$  is given by:

\begin{equation}\label{eq:ps.response.transform.erl}
(1-\rho)(1-\rho x^2)(\gamma k)^k \Phi\left(\dfrac{\rho(1-x)^2}{(1-\rho x)^2}, k, \dfrac{x(\lambda(1-x)+s+k\gamma)}{\mu(1-\rho x^2)} \right)
\end{equation}

where $\phi(z,b,a)$ is the Lerch Transcendent function.

\end{theorem}
\end{comment}

\subsection{Parameter Estimation}
Let us consider the case in which we have to differentiate between two classes of network requests  that we denote as class $0$ and class $1$. In order to estimate the parameters of the service and response time of the customers of these two types, we perform some preliminary measurements obtaining the response time for requests performed by a probe customer under different load conditions. From measurements we obtain:
\begin{itemize}
    \item $Y^{0} = (Y_1^{0}, Y_2^{0}, \dots, Y_{N^{0}}^{0})$: response times measured for requests of the probe customers under the lowest observed load factor
    %\item $X^{1} = (X_1^{1}, X_2^{1}, \dots, X_{N^{1}}^{1})$: response times measured for requests of class $1$ under the lowest observed load factor.
    \item $Y^{R} = (Y_1^{R}, Y_2^{R}, \dots, Y_{N^R}^{R})$: response times for requests of the probe customer under the most recent load factor.
\end{itemize}

Denote with $\xrv$ the service time of the probe customer. Assume that $\xrv$ results from the sum of two components: a constant $\erlshift$ and a variable $\vrv$. Suppose that $\vrv$ is a random variable with an Erlang distribution of $k$ stages and mean $1/\gamma$ expressed in the following manner
\begin{equation}
    \vcdf(t, k, \gamma) = Pr\{\vrv\leq t\} = 1 - \sum_{n=0}^{k-1} \dfrac{(k\gamma t)^n}{n!} e^{-k\gamma t}\,.
\end{equation}
$\xrv$ is thus a random variable whose Cumulative Distribution Function (CDF) can be expressed as follows:
\begin{align}\allowdisplaybreaks
    \xcdf(t, k, \gamma) &= Pr\{\xrv\leq t\} = \nonumber \\
    &\begin{cases}
        0 & t\leq \erlshift \\
        Pr\{\vrv\leq t-\erlshift\} = \vcdf(t-\erlshift, k, \gamma)  & t > \erlshift\,.
    \end{cases}
\end{align}

\begin{remark}
Recall that each of the $k$ stages of an Erlang distribution with expected value equal to $1/\gamma$ has a negative-exponential distribution with mean equal to $1/k\gamma$
\end{remark}



The parameters of the distribution of $\xrv$ can be estimated from the collection of the $N$ response time measures observed under the lowest load factor. Specifically, referring to the collection of observations denoted above with $Y^0$ and omitting the superscript to make the notation simpler, we can estimate the constant $\erlshift$ (i.e. the Erlang shift) and the parameters of the r.v. $\vrv$ ($\gamma$ and $k$) \textcolor{blue}{in the following way.\\
Let us first denote with 
 $\widehat{Y},\ \widehat{\sigma^2}(Y),\ \text{and},\ \widehat{\nu_0}(Y)$ the mean, variance and mode of the sample of observations $Y$.}\\
 
 We can state that
\[
E[\xrv] = C + E[\vrv] = C + \dfrac{1}{\gamma}\ \textcolor{blue}{\approx \widehat{Y}}\,,
\]
\ 
\[
\text{VAR}[\xrv] = \text{VAR}[\vrv] = \dfrac{1}{k\gamma^2}\ \textcolor{blue}{\ \approx \widehat{\sigma^2}(Y)}
\]
and
\[
\text{MODE}[\xrv]  = C + \text{MODE}[\vrv] \textcolor{blue}{\approx \widehat{\nu_0}(Y)}\,, 
\]
and thus obtain the desired quantities by solving the following system of equations
\[
\begin{cases}
    \widehat{\sigma^2}(Y) = \dfrac{1}{k\gamma^2} & \\
    \widehat{Y} = \dfrac{1}{\gamma} + \erlshift  & \\
    \widehat{\nu_0}(Y)=\dfrac{1}{k\gamma}(k-1)+\erlshift  & \\
\end{cases}
\]

The solution of this system of equations is given by:
\[
\begin{cases}
    k = \dfrac{\widehat{\sigma^2}(Y)}{(\widehat{Y}-\widehat{\nu_0}(Y))^2}  & \\\\
    \gamma = \dfrac{\widehat{Y}-\widehat{\nu_0}(Y)}{\widehat{\sigma^2}(Y)} & \\\\
    \erlshift = \widehat{Y} - \dfrac{\widehat{\sigma^2}(Y)}{\widehat{Y}-\widehat{\nu_0}(Y)} & \\
\end{cases}
\]
Notice that within these derivations, we assume that the $\{Y_i\}$ are measures of the service time of the probe customer only (i.e., under low load conditions, the waiting time for the processing of other requests is assumed to be negligible).
\textcolor{blue}{Moreover, notice that $k$ is by definition an integer quantity, while the expression given before provides a real result that must be rounded. For this reason it is convenient to observe that $\gamma$ and $C$ can be expressed in the following way
}
\[
\begin{cases}
    \gamma = \dfrac{1}{(\widehat{Y}-\widehat{\nu_0}(Y))\, k } & \\\\
    \erlshift = \widehat{Y} - (\widehat{Y}-\widehat{\nu_0}(Y))\, k & \\
\end{cases}
\]
\textcolor{blue}{so that $\gamma$ and $C$ are evaluated only after having computed the desired value of $k$.
}
\ \\



\textbf{\textcolor{red}{WHAT IF WE USE SKEWNESS INSTEAD OF MODE?}}

\ext{We can state that
\[
E[\xrv] = C + E[\vrv] = C + \dfrac{1}{\gamma}\ \textcolor{blue}{\approx \widehat{Y}}\,,
\]
\ 
\[
\text{VAR}[\xrv] = \text{VAR}[\vrv] = \dfrac{1}{k\gamma^2}\ \textcolor{blue}{\ \approx \widehat{\sigma^2}(Y)}
\]
and
\[
\text{SKEW}[\xrv]  = \text{SKEW}[\vrv] \textcolor{blue}{\approx \widehat{\kappa_3}(Y)}\,, 
\]
and thus obtain the desired quantities by solving the following system of equations
\[
\begin{cases}
    \widehat{\sigma^2}(Y) = \dfrac{1}{k\gamma^2} & \\
    \widehat{Y} = \dfrac{1}{\gamma} + \erlshift  & \\
    \widehat{\kappa_3}(Y)=\dfrac{2}{\sqrt{k}}  & \\
\end{cases}
\]

The solution of this system of equations is given by:
\[
\begin{cases}
    k = \dfrac{4}{(\widehat{\kappa_3}(Y))^2}  & \\\\
    \gamma = \dfrac{\widehat{\kappa_3}(Y)}{2\sqrt{\widehat{\sigma^2}(Y)}} & \\\\
    \erlshift = \widehat{Y} - \dfrac{2\sqrt{\widehat{\sigma^2}(Y)}}{\widehat{\kappa_3}(Y)} & \\
\end{cases}
\]}

To keep again the derivation simple, let us denote with $\rrv$ the response time of the probe customer under general loading conditions (i.e., $\rrv_i = Y_i^R$). We can define $\rrv = W + S$, where $W$ is the waiting (delay) time due to the processing
of other customer’s requests. \\
With this notation, and exploiting properties of conditional probabilities, we can express the probability of a zero waiting time under the condition of observing a response time for the probe customer under general load conditions.

In order to do so we first make the following observations:
\[
Pr\{\wrv=0 | \xrv=p,\ \rrv=q \} = \mathds{1}_{q\leq p}\,,
\]
we decondition with respect to the service time distribution
\begin{align*}
Pr\{\wrv=0 | \rrv=q \} &= \int_0^{\infty} \mathds{1}_{q\leq p} x(p) dp\\ &= \int_q^\infty f(p) dp = 1-\xcdf(q)\,,
\end{align*}
the last step consists of deconditioning with respect to the discrete amount of response time observations, so to obtain:
\begin{align*}
\widehat{Pr}\{\wrv=0\}&=1-\dfrac{1}{N^R}\sum_{i=1}^{N^R} \xcdf(\rrv_i, k, \gamma) \\ &= 1-\dfrac{1}{N^R}\sum_{i=1}^{N^R}\vcdf(\rrv_i - \erlshift, k, \gamma)\,.
\end{align*}

Now, recalling that in a M/M/1/PS queuing system, 
\begin{itemize}
\item
the expected response time of a customer with a service time equal to $\eta$ is 
\[
E[\rrv|\eta] = \dfrac{\eta}{1-\rho}\,,
\]
\ext{To find the average response time, $E[\rrv]$, we integrate this conditional expectation over the Erlang density of the service time
\begin{align*}
E[\rrv] &= \int_\erlshift^{\infty} E[\rrv\ |\ \eta] x(\eta-\erlshift)\ d\eta\,, \\
&= \int_\erlshift^{\infty} \dfrac{\eta}{1-\rho} x(\eta-\erlshift)\ d\eta\,, \\
&= \dfrac{1}{1-\rho}\int_\erlshift
^{\infty} \eta  \dfrac{k\gamma^k(\eta-\erlshift)^{k-1}e^{-k\gamma(\eta-\erlshift)}}{(k-1)!}\ d\eta\,, \\
&= \dfrac{C\gamma + 1}{\gamma(1-\rho)}\,, \\
\end{align*}
}
\item the probability of finding the system empty is
\[
\pi_0 = 1 -\rho\,,
\]
\item the probability of an incoming customer to have waiting time equal to 0 is:
\ext{
\begin{align*}
    &Pr\{\wrv=0\} = \\
    &= \int_\erlshift^{\infty} \pi_0e^{-\lambda\eta} x(\eta-\erlshift) d\eta\,,\\
    &= \pi_0\int_{\erlshift}^{\infty} e^{-\lambda\eta} x(\eta-\erlshift) d\eta\,,\\
    &= \pi_0\int_{\erlshift}^{\infty} e^{-\lambda\eta} \dfrac{(k\gamma)^k (\eta-\erlshift)^{k-1}e^{-k\gamma (\eta-\erlshift)}}{(k-1)!}d\eta\,,\\
    &= \dfrac{\pi_0(k\gamma)^k}{(k-1)!}\int_{\erlshift}^{\infty} e^{-\lambda\eta} (\eta-\erlshift)^{k-1}e^{-k\gamma (\eta-\erlshift)}d\eta\,,\\
    &\ \text{Let } u = \eta - \erlshift\\
    &= \dfrac{\pi_0(k\gamma)^k}{(k-1)!}\int_{0}^{\infty} e^{-\lambda(u+\erlshift)} u^{k-1}e^{-k\gamma u}du\,,\\
    &= \dfrac{\pi_0e^{-\lambda\erlshift}(k\gamma)^k}{(k-1)!}\int_{0}^{\infty} u^{k-1}e^{-(\lambda+k\gamma) u}du\,,\\
    &= \dfrac{\pi_0 e^{-\lambda\erlshift}(k\gamma)^k}{(k-1)!(\lambda + k\gamma)^{k-1}}\int_{0}^{\infty} (\lambda + k\gamma)u)^{k-1}e^{-(\lambda+k\gamma) u}du\,,\\
    &\text{Letting } t = (\lambda+k\gamma)u, \text{and thus } du =\dfrac{dt}{(\lambda + k\gamma)}\,,\\
     &= \dfrac{\pi_0 e^{-\lambda\erlshift}(k\gamma)^k}{(k-1)!(\lambda + k\gamma)^{k}}\int_{0}^{\infty} t^{k-1}e^{-t}dt\,,\\
     &\ \text{By def. of gamma function: } \Gamma(z)=\int_0^{\infty} t^{z-1} e^{-t}\ dt\,,\\
     &= \dfrac{\pi_0 e^{-\lambda\erlshift}(k\gamma)^k}{(k-1)!(\lambda + k\gamma)^{k}}\Gamma(k)\,,\\
    &= \pi_0 e^{-\lambda\erlshift} \left( \dfrac{k\gamma}{\lambda + k\gamma }\right) ^k\,.\\
\end{align*}
}
\end{itemize}
\ext{We can observe that in our case $E[\rrv]=\widehat{Y^R}$. On the basis of this observation, we obtain the estimated load factor as:
\[
\widehat{\rho} = 1- \dfrac{(1+\gamma \erlshift)}{\gamma\widehat{Y^R}}\,,
\]}
\begin{comment}
we can observe that in our case $\eta =\erlshift+1/ \gamma$ and $E[\rrv|\eta]=\widehat{Y^R}$.
On the basis of these observation, we obtain the estimated load factor as:
\[
\widehat{\rho} = 1- \dfrac{(1+\gamma \erlshift)}{\gamma\widehat{Y^R}}\,,
\]
\end{comment}
\ext{and the estimated the arrival rate as
\[
\widehat{\lambda}  = \dfrac{k}{\erlshift}\omega\left(\erlshift\gamma e^{\erlshift\gamma} \left(\dfrac{(1-\widehat{\rho})}{\widehat{Pr}\{\wrv=0\} }\right)^{\dfrac{1}{k}}\right) - k\gamma\,.
\]
from:
\begin{align*}
\widehat{Pr}\{\wrv=0\} &= (1-\widehat{\rho})e^{-\lambda\erlshift} \left( \dfrac{k\gamma}{\lambda + k\gamma }\right)^k\\
%\dfrac{\widehat{Pr}\{\wrv=0\} }{(1-\widehat{\rho})(k\gamma)^k} &=  \dfrac{1}{e^{\lambda\erlshift}(\lambda + k\gamma )^k} \\
e^{\lambda\erlshift}(\lambda + k\gamma )^k &= \dfrac{(1-\widehat{\rho})(k\gamma)^k}{\widehat{Pr}\{\wrv=0\} }\\
(\lambda + k\gamma )e^{\dfrac{\lambda\erlshift}{k}} &= k\gamma \left(\dfrac{(1-\widehat{\rho})}{\widehat{Pr}\{\wrv=0\} }\right)^{\dfrac{1}{k}}
\end{align*}
Now, we want the equation in the form $Z=Xe^ 
X$, so that we can apply Lambert-W function whose solution for $X$ is $\omega(Z)$ (computable in matlab).
\begin{align*}
&(\lambda + k\gamma )e^{\dfrac{\erlshift}{k}(\lambda+k\gamma - k\gamma)} = k\gamma \left(\dfrac{(1-\widehat{\rho})}{\widehat{Pr}\{\wrv=0\} }\right)^{\dfrac{1}{k}}\\
&(\lambda + k\gamma )e^{\dfrac{\erlshift}{k}(\lambda+k\gamma) - C\gamma} = k\gamma \left(\dfrac{(1-\widehat{\rho})}{\widehat{Pr}\{\wrv=0\} }\right)^{\dfrac{1}{k}}\\
&\underbrace{\dfrac{\erlshift}{k}(\lambda + k\gamma )}_{X}e^{\underbrace{\dfrac{\erlshift}{k}(\lambda+k\gamma)}_{X}} = \underbrace{\dfrac{\erlshift}{k}e^{\erlshift\gamma}k\gamma \left(\dfrac{(1-\widehat{\rho})}{\widehat{Pr}\{\wrv=0\} }\right)^{\dfrac{1}{k}}}_{Z}\\
&\dfrac{\erlshift}{k}(\lambda + k\gamma ) = \omega\left(\erlshift\gamma e^{\erlshift\gamma} \left(\dfrac{(1-\widehat{\rho})}{\widehat{Pr}\{\wrv=0\} }\right)^{\dfrac{1}{k}}\right)\\
&\lambda  = \dfrac{k}{\erlshift}\omega\left(\erlshift\gamma e^{\erlshift\gamma} \left(\dfrac{(1-\widehat{\rho})}{\widehat{Pr}\{\wrv=0\} }\right)^{\dfrac{1}{k}}\right) - k\gamma\\
\end{align*}

}

%\subsection{Sanity Check with Previous Methodology - Mode Shift}
%\input{firstexps_mode_shift_ps}
%\input{firstexps}

==> backup-dituttounpo/mm1ps_noshift.tex <==
\subsection{Response time distribution in M/M/1/PS with probe job}
\textcolor{blue} {Io qui' aggiungerei una prima descrizione qualitativa del metodo seguito per ottenere il risultato desiderato 
\begin{itemize}
\item richiamando e commentando minimamente il risultato di Muntz, Coffman etc\\
\item evidenziando la necessita' di completare quel risultato per ottenere il Response time
\item motivando la scelta di ottenere il risultato desiderato inserendo il probe job\
\item e quindi spiegando il ruolo dei corollari e del teorema\\
\end{itemize}
\ \\
\ \\
}
With a slight abuse of notation, we define the following expressions to facilitate the subsequent discussion.
\begin{align*}
    a &= \lambda(1-\muntzroot)\\
    b &= (1-\rho \muntzroot)^2\\
    g &= \rho (1-\muntzroot)^2\\
    h &= \dfrac{\mu (1-\rho \muntzroot^2)}{\muntzroot}
\end{align*}

where $\muntzroot$ is the smallest of the two positive roots of the equation
\[
\rho \muntzroot^2 - (\lambda + \mu + s) \muntzroot + \mu = 0
\]
The expression for $\muntzroot$ is the following
\[
\muntzroot = \dfrac{\lambda + \mu + s - [(\lambda+\mu+s)^2 - 4 \mu\lambda]^{1/2}}{2\lambda},\ \text{and}\ \rho=\dfrac{\lambda}{\mu}<1\,.
\]
Notice that $\lambda,\ \mu \in  \mathbb{R^+}$, moreover as stated in~\cite{morrison}, $0 < \muntzroot \leq 1,\ \text{for}\ s\geq 0\,.$


Let $\mathcal W_\eta$ be the r.v. associated with the stationary waiting time of a job whose service requirement is $\eta$.
From \cite[Corollary 1]{muntz-lstPSwaitTime} we know that under the stability condition $\rho<1$, the CDF of this r.v. can be expressed in the following way:
\[
\wcdf(\eta, t)=Prob\{\mathcal \wrv_\eta \leq t\}\,.
\]


Then, we can define the Laplace-Stieltjes transform:
\[
\wlst(\eta,s)\triangleq\int_0^\infty \exp(-s t) d_t\wcdf(\eta,t)
\]
of the equilibrium waiting time distribution conditioned on the job requiring $\eta$ units of service, namely  

\begin{equation}\label{eq:conditional.ps}
\wlst(\eta, s) = \dfrac{(1-\rho)(1-\rho \muntzroot^2)\exp(- a \eta)}{b - g \cdot \exp(-h\eta)}\,.
\end{equation}

with $\eta \in \mathbb R^+$ representing the deterministic service time of the probe job. 
Let $\rrv_\eta$ be the r.v. associated with a job of size $\eta$, and let $\rcdf(\eta,t)$ be the corresponding CDF defined as: 
\[
\rcdf(\eta,t)=
\begin{cases}
0 & \text{if }t < \eta \\
\wcdf(\eta, t-\eta) & t \geq \eta
\end{cases}
\]
i.e., the CDFs of $\rrv_\eta$ and $\wrv_\eta$ are the same modulo a shifting on the $t$-axis of width $\eta$.
\[
\wcdf(\eta, t) = \rcdf(\eta, t+\eta)\,, \quad t\geq \eta 
\]



Applying the \textit{time-shifting} property of Laplace transforms\footnote{Given the function $f(t)$ and its respective Laplace transform $f^*(s)$ we have that \[f(t-a)u(t-a)=\exp(-a s) f^*(s)\,.\]}, we obtain the Laplace transform of the response time, conditioned on the job requiring a service time $\eta$:
\begin{equation}\label{eq:shift}
\rlst(\eta, s) = \exp(-s \eta) \wpdf(\eta, s)\,.
\end{equation}
\begin{itemize}
\item \textcolor{red}{Chiarire bene che $\eta$ è una quantità deterministica, e $\tau$ invece è un parametro di una distribuzione, entrambi riferiti al service time del probe job}
\item \textcolor{red}{abbiamo la trasformata condsizionata su un $\tau$, poi passiamo a dare una distribuzione a questo probe job. Di fatto asusmiamo che questo probe job non alteri il funzionamento del sistema in quanto è un uno su infiniti, che arriva e vede il sistema come se lui non ci fosse e vede successivamente il sistema alterttando inalterato}
\end{itemize}
By the law of total probabilities we can decondition the expression above as follows:
\begin{equation}\label{eq:totprob}
    \rlst(s) = \int_0^\infty \rlst(\tau, s) d\xcdf(\tau)\,,
\end{equation}
where $\xcdf(\tau)$ is the CDF of the service time distribution of the probe job. 


\noindent Given the following definition

\begin{definition}
    The Lerch Trascendent function~\cite[Eq.~(25.14.1), pp. 612]{nist} is defined as:
    \[
    \Phi(z,u,\alpha) = \sum_{n=0}^{\infty} \dfrac{z^n}{(\alpha+n)^u}\,, \quad \text{with } |z|<1\,,
    \]
    which converges for any real number $\alpha>0$, where $|z|<1$, or $\mathrm{Re}(u) > 1$, and $|z| = 1$\,.
\end{definition}

\noindent we can state Theorem~\ref{th:probe-erl}.




\begin{theorem}\label{th:probe-erl}
    Given a M/M/1/PS (\textcolor{red}{NB. chiarire che caratterizzando il service time del probe job con una Erlang-k non stiamo andando a studiare una M/Erl/1/PS}) queueing system with $\rho < 1$, assume that a probe job has a service time distributed according to an Erlang-k r.v. \textcolor{red}{with $k\gamma$ being the rate at each Erlang phase, and the Erlang parameter and itself}. Then, the Laplace-Stieltjes transform of the probe job's response time is:
    \begin{equation}\label{eq:ps.response.transform.erl}
        \rlst(s) = (k\gamma)^k(1-\rho)(1-\rho \muntzroot^2) \dfrac{1}{bh^k}\Phi\left(\dfrac{g}{b}, k, \dfrac{s+a+k\gamma}{h}\right)
    \end{equation}
\end{theorem}

In order to prove Theorem~\ref{th:probe-erl}, we need to state and prove the following two lemmas.

\begin{lemma}\label{lem:geomseries}
\[
    \dfrac{1}{1-\dfrac{g}{b}\exp(-h\tau)} =\sum_{n=0}^{\infty} \left(\dfrac{g}{b}\exp(-h\tau)\right)^n\,,
\]
as $\left|\dfrac{g}{b}\exp(-h\tau)\right|<1$, by Lemma~\ref{lem:bcg1}, and since $h,\ \tau \in \mathbb{R}^+$\\
(\textcolor{red}{E' giusto che l'argomento della sommatoria in $n$ non dipenda da $n$?  Inoltre, dove usiamo il Lemma 1 nella dimostrazine del teorema 1?})

\end{lemma}
% trasformata waiting time
% essendo il R = W + tau posso fare shift nel tempo della trasformata e ottengo trasformata resp time
% ora con legge total prob decondiziono per ottenere R medio decondizionato e aggiungo tempo servizio esponenziale con parametro gamma (?) problemito ?

\begin{lemma}\label{lem:changeOfVar}
We have that
\[
\int_0^{\infty} t^{k-1} \exp(-p t)\ d t = \dfrac{\Gamma(k)}{p^k}
\]    
\end{lemma}
\begin{proof}
\begin{align*}
    \int_0^{\infty} t^{k-1} \exp(-p t)\ d t &= \int_0^{\infty} \left(\dfrac{u}{p}\right)^{k-1} \dfrac{\exp(-u)}{p} \ \ d u \\ &\quad \text{by variable change } u = p t\\
    &= \dfrac{1}{p^k} \int_0^{\infty} u^{k-1} \exp(-u)\ d u\quad \\ &\text{pulling out constant factors}\\
    &= \dfrac{\Gamma(k)}{p^k}\quad \text{by integral repr.}\\ &\text{of Gamma function}
\end{align*}
\end{proof}

We are now in the condition of proving Theorem~\ref{th:probe-erl} as follows.






\begin{definition}
    The Hypergeometric function~\cite[Eq.~(15.2.1), pp. 384]{nist}, $_2F_1(k,y;u;z)$ is defined as:
    \[
    _2F_1(m,p;u;z) = \sum_{n=0}^{\infty} \dfrac{(m)_n (p)_n}{(u)_n}\dfrac{z^n}{n!}\,, \quad \text{ with } |z|<1,\ u > 0,\ 
    \]
    with $(q)_n$ being the (rising) Pochhammer symbol\footnote{Pochhammer symbol $(q)_n$ is defined as follows:
    \[
    (q)_n = \begin{cases}
        1 & n =0\\
        q(q+1)\cdots (q+n-1) & n > 0
    \end{cases}
    \]} and considering it converges conditionally when $-1<\mathrm{Re}(u-m-p)\leq 0\,.$ and $z=1$ is excluded.
\end{definition}



\begin{comment}
\noindent Given the following definitions and :
\begin{itemize}
    \item the Lerch Trascendent function~\cite[Eq.~(25.14.1), pp. 612]{nist}:
    \[
    \Phi(z, v,y) = \sum_{n=0}^{\infty} \dfrac{z^n}{(y+n)^v}\,, \quad \text{with } |z|<1\,,
    \]
    which converges for any real number $y>0$, where $|z|<1$, or $\mathcal{R}(s) > 1$, and $|z| = 1$\,.
    \item the hypergeometric function~\cite[Eq.~(15.2.1), pp. 384]{nist}:
    \[
    _2F_1(k,y;v;z) = \sum_{n=0}^{\infty} \dfrac{(k)_n (y)_n}{(v)_n}\dfrac{z^n}{n!}\,, \quad \text{with} |z|<1,\ v > 0,\ 
    \]
    with $(q)_n$ being the (rising) Pochhammer symbol\footnote{Pochhammer symbol $(q)_n$ is defined as follows:
    \[
    (q)_n = \begin{cases}
        1 & n =0\\
        q(q+1)\cdots (q+n-1) & n > 0
    \end{cases}
    \]} and considering it converges conditionally when $-1<\mathcal{R}(v-k-y)\leq 0\,.$ and $z=1$ is excluded.
    % \item We also have:
    % \[
    % _2F_1(k, y;v, z) =\ _2F_1(y, k;v, z)\,, 
    % \]
    % by symmetry of the inferior indices.
    \item We also have a connection of the Lerch Trascendent function with the hypergeoemtric function:
    \[
    \Phi(z,1,y)=\dfrac{_2F_1(1, y, y+1, z)}{y}\,, \quad |z| < 1
    \]
    From~\cite[Eq.~(9.559), pp. 1039]{zwillinger2007table}
\end{itemize}
\end{comment}





\begin{result}\label{res:relationHyperLerch}
    We also have a connection of the Lerch Trascendent function with the hypergeomtric function:
    \[
    \Phi(z,1,\alpha)=\dfrac{_2F_1(1, \alpha, \alpha+1, z)}{\alpha}\,, \quad |z| < 1
    \]
    From~\cite[Eq.~(9.559), pp. 1039]{zwillinger2007table}
\end{result}

\begin{lemma}[Existance and Convergence]\label{lem:bcg1}      
The function
\[
_2F_1\left(1, \dfrac{a+\gamma +s}{h}; \dfrac{a+h+\gamma +s}{h}; \dfrac{g}{b} \right)
\]
exists and converges (conditionally) if and only if the following conditions are satisfied.
\[
\mathrm{(i)}\ \left|\dfrac{g}{b}\right| < 1\,,\ \mathrm{(ii)} \ \dfrac{s+a+\gamma+h}{h} > 0\,,\ 
\]
\[
\mathrm{(iii)}\ -1<\mathrm{Re}\left(\dfrac{s+a+\gamma+h}{h}-1-\dfrac{s+a+\gamma}{h}\right)\leq 0
\]
\end{lemma}
\begin{proof}
    We prove the three conditions separately.\\
    
    \noindent $\mathrm{(i)}$ $\left|\dfrac{g}{b}\right| < 1$\\
    \begin{align*}
        \dfrac{\rho(1-\muntzroot)^2}{(1-\rho \muntzroot)^2} &< 1\\
        \rho(1-\muntzroot)^2 &< (1-\rho \muntzroot)^2\\
        \rho(1-2\muntzroot+\muntzroot^2) &< (1-2\rho \muntzroot + \rho^2 \muntzroot^2) \\
        \rho +\rho \muntzroot^2 -1 -\rho^2 \muntzroot^2 &< 0\\
        \rho -1 + \rho \muntzroot^2 (1-\rho) &< 0\\
        (\rho -1) (1-\rho \muntzroot^2) &< 0
    \end{align*}
    since $0<\rho<1$, we have $(\rho -1)<0$, thus the inequality holds if 
    \[
    1-\rho \muntzroot^2 > 0,\quad  \text{i.e.,}\quad \muntzroot^2 <\dfrac{1}{\rho}
    \]
    as $0<\muntzroot\leq 1$ we need $1\leq \rho^{-1}$ which is always true for $0< \rho<1$. Thus, Condition (i) is satisfied.\\
    
    \noindent $\mathrm{(ii)}$ $\dfrac{s+a+\gamma+h}{h} > 0$\\
    \begin{itemize}
        \item[] $s\geq 0$, $\gamma > 0$
        \item[] $a = \lambda(1-\muntzroot)$, since $\lambda > 0$ and $0<\muntzroot\leq 1$ we obtain $a \geq 0$
        \item[] $h = \dfrac{\mu(1-\rho \muntzroot^2)}{\muntzroot}>0$, since $0<\muntzroot\leq 1$, $\mu > 0$, and $0<\rho<1$
    \end{itemize}
    Hence, condition $\mathrm{(ii)}$ is satisfied\\

    \noindent $\mathrm{(iii)}$ $\mathrm{Re}\left(\dfrac{s+a+\gamma+h}{h}-1-\dfrac{s+a+\gamma}{h}\right)\leq 0$\\
    
    After few algebraic steps we notice that the expression above is equal 0, thus condition (iii) is satisfied.\\
\end{proof}

\begin{corollary}\label{cor:mm1psexp}
    Given a M/M/1/PS queueing system with $\rho < 1 $, assume that a probe job has a service time distributed according to an Exponential r.v. Then, the Laplace-Stieltjes transform of the probe job's response time is:
    {\small
    \begin{equation}
        \rlst(s) = \dfrac{\gamma(1-\rho)(1-\rho \muntzroot^2)\ _2F_1\left(1, \dfrac{a+\gamma +s}{h}; \dfrac{a+h+\gamma +s}{h}; \dfrac{g}{b} \right)}{b(a+\gamma+s)}
    \end{equation}}
\end{corollary}



%Add here Muntz's result and our result on M/M/1/PS with probe job with Erlang service time distribution.
\begin{comment}
\begin{theorem}
Given a M/M/1/PS queueing system with $\rho<1$, assume that a probe job  has a service time distributed according to an Erlang-$k$ r.v.. Then, the Laplace-Stieltjes transform of the probe job's response time is:

\begin{multline}\label{eq:ps.response.transform}
\, _2F_1\left(1,\frac{x (\lambda (x-1)-s-\mu)}{\lambda x^2-\mu};-\frac{\mu + x (\lambda - 2 \lambda x + s + \mu)}{\lambda x^2 - \mu};\frac{\lambda (x-1)^2 \mu}{(\mu-\lambda x)^2}\right)\\ \cdot \frac{1}{(1-x \rho)^2 (\lambda(1-x)+s+u)}
\end{multline}


\begin{multline}\label{eq:ps.response.transform.exp}
\, _2F_1\left(1,\frac{x (\lambda (x-1)-s-\mu)}{\lambda x^2-\mu};-\frac{\mu + x (\lambda - 2 \lambda x + s + \mu)}{\lambda x^2 - \mu};\frac{\lambda (x-1)^2 \mu}{(\mu-\lambda x)^2}\right)\\ 
\cdot \dfrac{(1-\rho)(1-\rho x^2)\mu}{(1-x \rho)^2 (\lambda(1-x)+s+u)}
\end{multline}
When $k=1$, i.e. when the Erlang distribution collapses in an exponential distribution. The LST of the probe job's response time with an arbitrary number of phases $k$  is given by:

\begin{equation}\label{eq:ps.response.transform.erl}
(1-\rho)(1-\rho x^2)(\gamma k)^k \Phi\left(\dfrac{\rho(1-x)^2}{(1-\rho x)^2}, k, \dfrac{x(\lambda(1-x)+s+k\gamma)}{\mu(1-\rho x^2)} \right)
\end{equation}

where $\phi(z,b,a)$ is the Lerch Transcendent function.

\end{theorem}
\end{comment}

\subsection{Parameter Estimation}
Let us consider the case in which we have to differentiate between two classes of network requests  that we denote as class $0$ and class $1$. In order to estimate the parameters of the service and response time of the customers of these two types, we perform some preliminary measurements obtaining the response time for requests performed by a probe customer under different load conditions. From measurements we obtain:
\begin{itemize}
    \item $Y^{0} = (Y_1^{0}, Y_2^{0}, \dots, Y_{N^{0}}^{0})$: response times measured for requests of the probe customers under the lowest observed load factor
    %\item $X^{1} = (X_1^{1}, X_2^{1}, \dots, X_{N^{1}}^{1})$: response times measured for requests of class $1$ under the lowest observed load factor.
    \item $Y^{R} = (Y_1^{R}, Y_2^{R}, \dots, Y_{N^R}^{R})$: response times for requests of the probe customer under the most recent load factor.
\end{itemize}

Denote with $\xrv$ the service time of the probe customer. \noshift{Assume that $\xrv$ results from a random variable distributed according to a Erlang distribution of $k$ stages and mean $1/\gamma$ expressed in the following manner
\begin{equation}
    \xcdf(t, k, \gamma) = Pr\{\xrv\leq t\} = 1 - \sum_{n=0}^{k-1} \dfrac{(k\gamma t)^n}{n!} e^{-k\gamma t}\,.
\end{equation}}


\begin{remark}
Recall that each of the $k$ stages of an Erlang distribution with expected value equal to $1/\gamma$ has a negative-exponential distribution with mean equal to $1/k\gamma$
\end{remark}



The parameters of the distribution of $\xrv$ can be estimated from the collection of the $N$ response time measures observed under the lowest load factor. Specifically, referring to the collection of observations denoted above with $Y^0$ and omitting the superscript to make the notation simpler, \noshift{we can estimate the parameters of the r.v. $\vrv$ ($\gamma$ and $k$) in the following way.\\
Let us first denote with 
 $\widehat{Y},\ \widehat{\sigma^2}(Y)$ the mean, and the variance of the sample of observations $Y$.}\\
 
\noshift{We can state that
\[
E[\xrv] = \dfrac{1}{\gamma}\ \approx \widehat{Y}\,,
\]
\ 
\[
\text{VAR}[\xrv] = \dfrac{1}{k\gamma^2}\ \ \approx \widehat{\sigma^2}(Y)
\]
and thus obtain the desired quantities by solving the following system of equations
\[
\begin{cases}
    \widehat{\sigma^2}(Y) = \dfrac{1}{k\gamma^2} & \\
    \widehat{Y} = \dfrac{1}{\gamma}   & \\
\end{cases}
\]}

\noshift{The solution of this system of equations is given by:
\[
\begin{cases}
    k = \dfrac{\widehat{Y}^2}{\widehat{\sigma^2}(Y) } & \\\\
    \gamma = \dfrac{1}{\widehat{Y}} & \\\\
\end{cases}
\]
Notice that within these derivations, we assume that the $\{Y_i\}$ are measures of the service time of the probe customer only (i.e., under low load conditions, the waiting time for the processing of other requests is assumed to be negligible).
\textbf{Moreover, notice that $k$ is by definition an integer quantity, while the expression given before provides a real result that must be rounded.}}


To keep again the derivation simple, let us denote with $\rrv$ the response time of the probe customer under general loading conditions (i.e., $\rrv_i = Y_i^R$). We can define $\rrv = W + S$, where $W$ is the waiting (delay) time due to the processing
of other customer’s requests. \\
With this notation, and exploiting properties of conditional probabilities, we can express the probability of a zero waiting time under the condition of observing a response time for the probe customer under general load conditions.

In order to do so we first make the following observations:
\[
Pr\{\wrv=0 | \xrv=p,\ \rrv=q \} = \mathds{1}_{q\leq p}\,,
\]
we decondition with respect to the service time distribution
\begin{align*}
Pr\{\wrv=0 | \rrv=q \} &= \int_0^{\infty} \mathds{1}_{q\leq p} x(p) dp\\ &= \int_q^\infty f(p) dp = 1-\xcdf(q)\,,
\end{align*}
the last step consists of deconditioning with respect to the discrete amount of response time observations, \noshift{so to obtain:
\begin{align*}
\widehat{Pr}\{\wrv=0\}&=1-\dfrac{1}{N^R}\sum_{i=1}^{N^R} \xcdf(\rrv_i, k, \gamma)
\end{align*}}

Now, recalling that in a M/M/1/PS queuing system, 
\begin{itemize}
\item
the expected response time of a customer with a service time equal to $\eta$ is 
\[
E[\rrv|\eta] = \dfrac{\eta}{1-\rho}\,,
\]
\noshift{To find the average response time, $E[\rrv]$, we integrate this conditional expectation over the Erlang density of the service time
\begin{align*}
E[\rrv] &= \int_0^{\infty} E[\rrv\ |\ \eta] x(\eta)\ d\eta\,, \\
&= \int_0^{\infty} \dfrac{\eta}{1-\rho} x(\eta)\ d\eta\,, \\
&= \dfrac{1}{1-\rho}\underbrace{\int_0
^{\infty} \eta  \dfrac{(k\gamma)^k\eta^{k-1}e^{-k\gamma\eta}}{(k-1)!}}_{E[\xrv]}\ d\eta\,, \\
&= \dfrac{1}{\gamma(1-\rho)}\,,
\end{align*}
}
\item the probability of finding the system empty is
\[
\pi_0 = 1 -\rho\,,
\]
\item the probability of an incoming customer to have waiting time equal to 0 is:
\noshift{
\begin{align*}
    &Pr\{\wrv=0\} = \\
    &= \int_0^{\infty} \pi_0e^{-\lambda\eta} x(\eta) d\eta\,,\\
    &= \pi_0\int_{0}^{\infty} e^{-\lambda\eta} x(\eta) d\eta\,,\\
    &= \pi_0\int_{0}^{\infty} e^{-\lambda\eta} \dfrac{(k\gamma)^k \eta^{k-1}e^{-k\gamma \eta}}{(k-1)!}d\eta\,,\\
    &= \dfrac{\pi_0(k\gamma)^k}{(k-1)!}\int_{0}^{\infty} e^{-\lambda\eta} \eta^{k-1}e^{-k\gamma \eta}d\eta\,,\\
    &= \dfrac{\pi_0(k\gamma)^k}{(k-1)!}\int_{0}^{\infty}\eta^{k-1}e^{-(\lambda+k\gamma) \eta}d\eta\,,\\
    &= \dfrac{\pi_0(k\gamma)^k}{(k-1)!(\lambda + k\gamma)^{k-1}}\int_{0}^{\infty}((\lambda+k\gamma)\eta)^{k-1}e^{-(\lambda+k\gamma) \eta}d\eta\,,\\
    &\ \text{Let } t = (\lambda + k\gamma)\eta, \text{so that } \eta = \dfrac{t}{\lambda + k\gamma}\\
    &= \dfrac{\pi_0(k\gamma)^k}{(k-1)!(\lambda + k\gamma)^{k-1}}\int_{0}^{\infty}t^{k-1}e^{-t}d\dfrac{t}{\lambda+k\gamma}\,,\\
    &= \dfrac{\pi_0(k\gamma)^k}{(k-1)!(\lambda + k\gamma)^{k}}\int_{0}^{\infty}t^{k-1}e^{-t}dt\,,\\
    &= \dfrac{\pi_0(k\gamma)^k\Gamma(k)}{(k-1)!(\lambda + k\gamma)^{k}}\,,\\
    &= \pi_0\left(\dfrac{k\gamma}{\lambda + k\gamma}\right)^{k}\,,
\end{align*}
}
\end{itemize}
\noshift{We can observe that in our case $E[\rrv]=\widehat{Y^R}$. On the basis of this observation, we obtain the estimated load factor as:
\[
\widehat{\rho} = 1- \dfrac{1}{\gamma\widehat{Y^R}}\,,
\]}
\noshift{and the estimated arrival rate as
\[
\widehat{\lambda}  = k\gamma \left[\left(\dfrac{1-\widehat{\rho}}{\widehat{Pr}\{\wrv=0\}}\right)^{\dfrac{1}{k}}-1\right]\,.
\]
from:
\begin{align*}
\widehat{Pr}\{\wrv=0\} &= (1-\widehat{\rho})\left( \dfrac{k\gamma}{\lambda + k\gamma }\right)^k\\
\dfrac{\widehat{Pr}\{\wrv=0\}}{1-\widehat{\rho}} &= \left( \dfrac{k\gamma}{\lambda + k\gamma }\right)^k\\
\left(\dfrac{\widehat{Pr}\{\wrv=0\}}{1-\widehat{\rho}}\right)^{1/k} &= \left( \dfrac{k\gamma}{\lambda + k\gamma }\right)\\
\lambda+k\gamma &= k\gamma \left(\dfrac{1-\widehat{\rho}}{\widehat{Pr}\{\wrv=0\}}\right)^{1/k}\\
\lambda &= k\gamma \left[\left(\dfrac{1-\widehat{\rho}}{\widehat{Pr}\{\wrv=0\}}\right)^{\dfrac{1}{k}}-1\right]\,.
\end{align*}

}

%\subsection{Sanity Check with Previous Methodology - Mode Shift}
%\input{firstexps_mode_shift_ps}
%\input{firstexps}

==> backup-dituttounpo/models_comparison.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{3}{c}{DET} & \multicolumn{3}{c}{CONT} & \multicolumn{3}{c}{FCFS}  & \multicolumn{3}{c}{SOTA} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
Site & TPR & TNR & AR & TPR & TNR & AR & TPR & TNR & AR & TPR & TNR & AR \\
\midrule
bing & 0.000 & 0.000 & 0.938 & 1.000 & 0.000 & 0.750 & 0.000 & 1.000 & 0.375 & 0.000 & 0.000 & 1.000 \\
facebook & 1.000 & 1.000 & 0.312 & 1.000 & 1.000 & 0.250 & 1.000 & 1.000 & 0.438 & 1.000 & 1.000 & 0.188 \\
office & 0.875 & 0.875 & 0.000 & 1.000 & 1.000 & 0.188 & 0.625 & 1.000 & 0.000 & 0.500 & 0.667 & 0.438 \\
pinterest & 1.000 & 0.875 & 0.000 & 1.000 & 1.000 & 0.188 & 0.125 & 1.000 & 0.000 & 0.833 & 1.000 & 0.313 \\
spotify & 1.000 & 0.875 & 0.000 & 0.000 & 1.000 & 0.062 & 0.000 & 1.000 & 0.000 & 1.000 & 1.000 & 0.750 \\
\midrule
Average & 0.775 & 0.725 & 0.250 & 0.800 & 0.800 & 0.288 & 0.350 & 1.000 & 0.163 & 0.667 & 0.733 & 0.538 \\
\bottomrule
\end{tabular}
\caption{Comparison of PS deterministic, PS continuous, and FCFS models.}
\label{tab:cross_site_summary}
\end{table}
